When Tables Go Crazy: Evaluating Multimodal Models on French Financial Documents

Vision-language models (VLMs) perform well on many document understanding tasks, yet their reliability in specialized, non-English domains remains underexplored. This gap is especially critical in finance, where documents mix dense regulatory text, numerical tables, and visual charts, and where extraction errors can have real-world consequences. We introduce Scribe Finance, the first multimodal benchmark for evaluating French financial document understanding. The dataset contains 1,204 expert-validated questions spanning text extraction, table comprehension, chart interpretation, and multi-turn conversational reasoning, drawn from real investment prospectuses, KIDs, and PRIIPs. We evaluate six open-weight VLMs (8B-124B parameters) using an LLM-as-judge protocol. While models achieve strong performance on text and table tasks (85-90% accuracy), they struggle with chart interpretation (34-62%). Most notably, multi-turn dialogue reveals a sharp failure mode: early mistakes propagate across turns, driving accuracy down to roughly 50% regardless of model size. These results show that current VLMs are effective for well-defined extraction tasks but remain brittle in interactive, multi-step financial analysis. Scribe Finance offers a challenging benchmark to measure and drive progress in this high-stakes setting.

==> new_dataset_construction.tex <==
\subsection{Dataset Collection}

% Je pense qu'il faut changer cette phrase. Les reviewers ont pensés qu'il y avait une phase d'annotation plus importante qu'en réalité

Designing \ScribeFinance required balancing realism, scale, and annotation reliability. French financial prospectuses are long, repetitive, and highly structured documents that combine dense legal text with tables and charts, often spanning hundreds of pages. Rather than treating these documents as monolithic inputs, we focus on evaluating a model’s ability to accurately locate and extract specific, document-grounded information-a prerequisite for reliable downstream reasoning in financial settings.

% to evaluate a model’s ability to retrieve and interpret relevant financial information across heterogeneous inputs.

The dataset was constructed from publicly available French financial documents collected from multiple asset management companies, including prospectuses, KIDs, and PRIIPs published over the past 15 years. These documents cover a wide range of investment products and regulatory disclosures. In total, the dataset contains 1,204 questions, including 501 open-ended, 248 yes/no, 33 true/false, and 65 multiple-choice questions, as well as a subset of multi-turn conversational questions.
% 501+248+33+65 = 847 somethings wrong

Question construction followed an iterative, semi-automatic process designed to identify salient, extractable financial information. Large language models (GPT-4o and Gemini-2.0) were used to assist in question and answer generation, with all generated content subsequently reviewed and revised by human annotators. During this process, input contexts were expanded when necessary to ensure completeness, clarity, and faithful grounding in the source documents.

A deliberate design choice was made to anchor each question to a specific document excerpt rather than relying on full-document inputs. Given the size and redundancy of many prospectuses, accurate information retrieval often requires precise localization within dense content. This design emphasizes retrieval accuracy as a core evaluation objective rather than assuming perfect access to relevant information.

Approximately half of the documents consist primarily of textual content, while the remainder include structured elements such as tables and charts. Tables were preserved and converted into structured tabular formats to enable reasoning over mixed textual and numerical inputs. For questions involving charts and other graphical elements, the original visual representations were retained and used directly during question construction.

Multi-turn conversational questions were created to evaluate model behavior across dialogue turns. In these settings, answers may depend on prior exchanges rather than being explicitly present in the immediate input context, requiring models to maintain consistency and coherence over multiple turns.

\subsection{Task Overview and Dataset Composition}

The benchmark comprises six task categories reflecting common financial document understanding scenarios. With the exception of text-only questions, all tasks involve multimodal inputs, where a relevant image (e.g., a table, chart, or document page) is provided alongside the textual context.



The task categories include: 
\begin{itemize}
    \item \textbf{Text Question}, focusing on extraction from purely textual contexts;
    \emph{«~Ce fonds est-il géré activement ou suit-il un indice de manière passive ?~»}
    \item \textbf{Table Comprehension}, requiring reasoning over structured tabular data; 
    \emph{«~À combien s'élèvent les frais courants annuels prélevés par le FCPE ?~»}
    \item \textbf{Chart Interpretation}, based on graphical financial representations;
    \emph{«~Combien de périodes consécutives sans cristallisation sont visibles sur le graphique ?~»} 
    \emph{«~Les frais d'entrée et de sortie sont-ils inclus dans le calcul des performances passées ?~»}
    \emph{«~Quelle est la seule année où la performance du fonds et celle de l’indice sont quasiment identiques ?~»}
    \item \textbf{Special Cases}, involving nuanced terminology or implicit reasoning; and two conversational settings;
    \emph{«~Quels instruments dérivés spécifiques peuvent être utilisés par le compartiment ?~»}
    \item \textbf{Conversational (Gold Context)} and \textbf{Conversational (Model Context)}, which differ in whether previous turns use oracle answers or model-generated predictions, enabling the study of error propagation.
% Add a link, the example is in the annexes
\end{itemize}  

% 120 questions ont été oubliées : ce sont les questions reformulées dans un style oral \textbf{conversationally rephrased yes/no questions} reflect realistic user questions, for example: \emph{«~Est-ce que ça coûte quelque chose pour quitter le fonds ?~»} and \emph{«~Faut en prendre au moins 10 pour l’action F au début ?~»}.

To capture a range of retrieval and reasoning challenges, tasks vary along two primary axes: \textbf{context length}, ranging from short excerpts to document-level inputs, and \textbf{context modality}, including plain text, tables, charts, and mixed formats. Questions are formulated in open-ended, binary (yes/no, true/false), and multiple-choice formats depending on the task.


\subsection{Dataset Statistics}
Table~\ref{tab:distribution} summarizes the distribution of questions across task categories, question types, and context modalities. The dataset includes both text-based and image-based questions, with open-ended formats dominating overall, while binary and conversational formats target more constrained reasoning settings.

Context lengths range from short passages (1--2 sentences) to full documents spanning multiple pages. The conversational subset consists of multi-turn dialogues of 5--10 exchanges, explicitly designed to probe error propagation and robustness in interactive scenarios.

